Investigations on Increased Data rate Differential Space-Time Block Codes for Single Carrier Wireless Systems

In this thesis, we study differential modulation schemes which do not need channel knowledge at the transmitter nor at the receiver. First, we consider single-antenna systems and investigate the use of Differential Amplitude Phase Shift Keying (DAPSK) modulation. We study the use of Multiple-Symbol Differential Detection (MSDD) to bridge the performance gap between coherent and non-coherent systems and remove the error floor associated with fast-fading channels. Second, we consider multi-antenna systems to combat fading and improve the transmission reliability. The resulting performance improvement (known as diversity) does not require additional bandwidth nor power. Achieving diversity using multiple antennas at the receiver (receive diversity) is proved to be a much simpler task than using multiple antennas at the transmitter (transmit diversity). However, in downlink mobile communications, mounting multiple antennas on the receiving mobile handsets results in an increase in the size and cost of mobiles. This motivates the need of transmit diversity, which can be achieved by a technique known as Space-Time Coding (STC). In this thesis, we investigate a class of ST codes known as Orthogonal Space-Time Block Codes (OSTBC), which achieves a good performance with linear decoding complexity. As an attempt to increase the data rate, the orthogonality requirement of OSTBCs is relaxed leading to the so-called Quasi-Orthogonal STBCs (QOSTBC). Recently a new class of QOSTBCs known as Minimum Decoding Complexity QOSTBCs (MDC-QOSTBC) has proved to increase the data rate with the same complexity requirement of OSTBCs. In this thesis, we propose the use of MDC-QOSTBC in differential non-coherent systems and show that their performance is remarkably better than that of differential OSTBCs.

==> Draft.tex <==
\chapter{Draft}
\label{Draft}
 %some code may be useful later
 % included in the ittuu template
 \begin{table}
\caption{Time Required for Calculation.}
\centering
\label{distrarch:tab:time_sum}
\end{table}

\include{DPSK_and_DAPSK}
 \begin{figure}[htp]
  \centering
		\includegraphics[width=0.6\textwidth]{ring_ratio_search_awgn_2DPSK_4DASK}                
  \caption{ring_ratio_search_awgn_2DPSK_4DASK}
  \label{fig:ring_ratio_search_awgn_2DPSK_4DASK}
\end{figure}

\newcommand{\newln}{\\&\quad\quad{}}



==> Hints.tex <==
In paper "`"'Novel Rotated Quasi-Orthogonal Space-Time Block Codes with the Fixed Nearest Neighbor Number 
I like the explanation and the way of referencing...You may use it in explaining the literature review. 
I like his way in saying, we have M Tx antennas, on every time slot -usually called channel use- each antenna is fed a symbol...

*** Hochwald proved that good codes for a coherent detection receiver are also good for a non-coherent receiver, so all codes designed in the literature for the coherent case can also be used for the non-coherent receiver.
In the SISO part you should mention
1- The use of the phase e(jtheta) in the model is to account for the AWGN channel, since the model serves as a general model for AWGN & Rayleigh fading channel.
2- Mention the work done using a twisted constellation of DAPSK and whether it provides any improvement compared to the independent amplitude phase modulation. Also mention that the advantage of the considered DAPSK is the independent amplitude and phase modulation.

You have to mention who are the leaders of each area, like Rohling is the one who introduced the DAPSK constellation & in which year, also same for STBC mention clearly the classification of STC into STBC and STTC and that STTC achieves higher diversity order but also results in higher complexity compared to STBC. Mention who started STM (Alamouti) without giving the name of Space time coding, but for 2 antennas only. Later Tarokh & Jafarkhani extended Alamouti's work to multiple antennas, and gave it the name (coined it the term) Space time coding. ....proved that only in the 2 antennas case, the code achieves full rate without sacrificing the diversity, since it is an OSTBC which achieves the maximum diversity order (r=M). For M>2 one either sacrifice the rate but still with max. diversity (since it is orthogonal) an example for this is the code proposed by Tirkkonen & Hotinnen, or one sacrifies the diversity for a higher rate.
To extend the work to Differnetial modulation, Hochwald proved that if a code has good performance with coherent detection, then it will also be good for use in non-coherent receivers. So alamouti's code (M=2, T'=2) and Tirkkonen-Hottinen code (M=4, T'=4) can be easily extended to the non-coherent case. However we have two questions now, 1- For differential modulation, we perform the fundamental Differential transmitter equation St=Vt*St_1, so for St and St_1 to have the same dimension, Vt must be square, so in this context we can not extend the coherent codes with rectanular structure (M != T'), so we should search a way out. 2- We want to include Amplitude modulation in the structure, using DAPSK symbols instead of DPSK symbols, when I tried to get the metric in the alamouti's code (M=2, T'=2) and Tirkkonen-Hottinen code (M=4, T'=4) cases, I found out that the decision can not be split among the K coded symbols, and this is a significant disadvantage, because one of the main advantages of OSTBC is the possibilty of splitting the decision over the different coded symbols [x1, x2 ....xK], and avoid the need of joint detection..so again I need a way out of this either a mathematical trick, or a mathematical approximation. I should be also trying the GLRT metric for the DAPSK MIMO case. I am currently considering only the Rayleigh block fading case.
While searching on "Differential space time block code with amplitude modulation"
I found an unaccessble paper entitled "Quadrature Amplitude Modulation for Differential Space-Time Block Codes" under http://portal.acm.org/citation.cfm?id=1555995
BTW as I have seen for example in the paper "Differential Space Time Block Codes Using Nonconstant Modulus Constellations" & in other papers,
it is always mentioned that having a larger distance in the constellation always accounts for gain in the BER performance eventhough I know that the Euclidean distance is not the measure in the differential modulation case, so for this you have to explain why the twisted constellation doesn't result in any imporovement if it really doesn't.
I may also include the advantage of using STFC instead of STBC. 
- By including receive diversity, we increased the diversity order which is (DO=nt*nr) & consequently the diversity gain,and the BER curves slope gets higher.
so far mentioned= aforementioned
In USTM the signals transmitted by the different antennas are mutually orthogonal.
- Multiple antennas has been a promising solution for increasing the system capacity.
- Paper ""Differentially en/decoded orthogonal space time block codes with APSK signals" (is a good paper to read), it mentions that Differential Space time coding has been proposed by Hochwald & Sweldens & independently by Hughs. In the paper it is also mentioned that Tarokh & Jafarkhani extended Alamouti's work to multiple antennas, and also to Differential PSK modulation in OSTBC.
Note it is always called Hermitian transpose and not just hermitian
As I have seen so far in the papers, when they consider the OSTBC, we know that the ML decision can be split over the different transmit symbols for example we decide on x1 & x2 independently in decoding Alamouti's code. This is always named as linear processing in the detection. I have also seen it named as fast ML decoding.
As mentioned, So in not necessarily I but we say So is arbitrary fixed Unitary matrix. It's very nice to say in the same paper, "kn is encoded from the log2(M) information bits.. Note the transmitted signal is root rho S, this is really important to explain in words what does the equation say, & emphasize that the transmitted signal is not S but root rho S. It is also useful to consider rho as the signal power and No as the noise power density, rather than considering rho as the signal to noise ratio and N0=1.

Also a good reference to read and gain main concepts of is saved in C:\Local Disk E\C-tech\Master project\papers named "Introduction to Space time coding". It is a very good document highlitening the most important concepts in STCs with illustractive examples. Worth reading 
For example one sentence I used to like to make sure of is in page 10 pdf saying
MIMO increases the channel capacity of a system, "This increase in channel capacity is known as multiplexing gain"
Also the info that the distribution of the input signal X that maximizes the channel capacity was proved to be "The Gaussian distribution".
Also see page 9 pdf, when the design criteria of codes was proved through the PEP, it was clearly mentioned that "`The slope of the bound (I assume also of BER) is the prduct of the number of receive antennas and the rank of the difference matrix". The diversity gain is defined to be the minumum of such rank over all code pairs. Also the coding gain is defined & compared to diversity gain as in the studien arbeit. Diversity gain is the rate of decrease of BER with SNR (hence the slope of the BER curve), where as the coding gain is the horizontal shift of the BER curve.
As mentioned in page 13, and as we have seen in DUSTM for Hochwald, we know that the design citeria is the worst PEP which reflects the effect of the siatnce spectrum On error probability.
p.13 In order to optimize the error performance, the number of possible transmit matrices L must be less than 2MT & the matrices can be designed to be orthogonal, whereas for optimal capacity, K=2MT and the modulation matrices are not orthogonal.

 Here http://circle.ubc.ca/handle/2429/15339 is an abstract of a master thesis similar to mine that aims at including amplitude modulation for a better performance in STC. It is very important to reread the abstract, it points out the advantage of creating STC from group structre mainly in that it can be extended to any number of antennas achieveing full rate & full diversity, where as in the OSTBC only Alamouti's code with two antennas can achieve full rate, plus the transmission in general cannot be generalized to mulitple antennas. Having said that, it is still not an easy task to find groups with achieve good performance, so this requires exhaustive computer search. Also the extension to higher spectral efficiency in bits/s/Hz where as in OSTBC one can increase the spectral efficiency by just considering higher order modulation.
 __
 By the way, I have seen in the papers, they call the detection of OSTBC which splits the decision for the different symbols each based on a ML decision, they call it a "Fast ML decoding"
 "Unitary Space–Time Codes From Alamouti's Scheme With APSK Signals" is also a good paper to refer to while writing enshaAllah. In this paper they define the diversity product as that defined by Hochwald as minimum of all codeword pairs of the sqrt of the determinant of the difference matrix, this is analogous to the coding gain as defined in the studien thesis. Calling it coding gain or diversity product, this is the used design criteria for full rank codes, like OSTBC. Full rank means that that the rank of all difference matrices equal the number of transmit antennas.
 
 Also if you go to goole books and search for books on Differential space Time code
 In the book named "" under http://books.google.com/books?id=_tDVrzdF6mUC&pg=PA195&dq=Differential+space+time+coding&hl=en&ei=-tdpTNm1DMvn4AbD4YnJCQ&sa=X&oi=book_result&ct=result&resnum=3&ved=0CDkQ6AEwAg#v=onepage&q=Differential%20space%20time%20coding&f=false
 chaper 8 page 195 is a very good explanation of the coherent detection description & assumptions & going to the Differential transmission for noncoherent detection
 * when you want to refer to a paper & the papers in this paper you say something like.......This is explained in detail in [1] and the references therein.
 In the same book (Differential space-time modulation) you see useful explanation (chapter 8)
 - Independent decision on the different PSK symbols of a STBC, is also termed as "decoupling" of the data symbols as explained in "Diffferential Space-Time Codes" by Tao. ( It is a good paper, use it for the main concepts & for documentation.
 - As in the same last mentioned paper, and as in many other papers, the cyclic (diagonal) codea proposed by Hochwald, they are termed DUSTM, where as codes which use PSK symbols in the matrix elements are termed DOSTBC.
 In the same paper it was mentioned that Tarokh proved in his paper "Space-Time Block Codes from Orthogonal designs", that full rate codes are achieved for M (Tx antennas)=2,4,8 for read valued symbols, and only for M=2 for complex valued symbols
 -____
 -Note that the APSK constellation is also called circular QAM (see http://en.wikipedia.org/wiki/Quadrature_amplitude_modulation)
 I like the part of Quantized QAM saying, Since QAM is usually square, some of these are rare—the most common forms are 16-QAM, 64-QAM, 128-QAM and 256-QAM. By moving to a higher-order constellation, it is possible to transmit more bits per symbol. However, if the mean energy of the constellation is to remain the same (by way of making a fair comparison), the points must be closer together and are thus more susceptible to noise and other corruption; this results in a higher bit error rate and so higher-order QAM can deliver more data less reliably than lower-order QAM, for constant mean constellation energy.
 Then in the same article "Also, the error-rate performance of 8-QAM is close to that of 16-QAM (only about 0.5 dB better[citation needed]), but its data rate is only three-quarters that of 16-QAM."
 For Quasi Orthogonal codes, refer to http://users.ece.utexas.edu/~rheath/courses/mimo/suggested_readings/ref/10-1.pdf
 
http://arxiv.org/ftp/cs/papers/0605/0605095.pdf is like a Journal paper, includes same technique of Tao of DOSTBC-QAM but with illustration, probably useful for documentation

So far I have seen people sometimes use SER instead of BER in their curves. I believe it is not just a matter of that they love using SER instead of BER. One main difference is that in our decision metric, we decide on a symbol, if the mertic results in a correct decision it means we decided correctly on the symbol, otherwise we decide on a symbol other than the one transmitted. So SEr tells us how often our metric works. Going from SER to BER, means mapping the decided symbol to its corresponding bit sequence, so BEr includes the effect of the quality of the bit-to-symbol mapping. Optimally the bit-to-symbol mapping should be such that the symbols that are most probable to be mistaken by each other should be assigned bit sequences that are as close as possible (minimum Hamming distance in the constellation). In the coherent transmission such symbols having the minimum Euclidean distance in the constellation, so the Euclidean distance is the measure of how probable the symbols may be mistaken. However in the non-coherent transmission, the distance measure is different and determined by the metric used. For this, a bit-to-symbol mapping other than thr gray code (optimal for the coherent case) should be used. It is not yet known what is the optimum bit to symbol mapping for the noncoherent case. To exclude the effect of the bit to symbol mapping, one can use the SER instead of the BER as the performance measure of the metric only. From the whole transmission perspective, what matters is how many bits arrived correct, so the BER takes into account the performance of all parts of the communication model. Similarly the Block error Rate (BLER) is useful for usage if the metric decides on a block as a whole (as in the cyclic/diagonal code case), not symbol by symbol ( as in the OSTBC case), so to compare only how often the metric succeed to decide on the sent symbol, we must use the BLER, probably that's why Tao used the BLER when comparing the cyclic code curves with his OSTBC-QAM.
One more worth mentioning thing is when it comes to comparing results of different techniques, it's better to use the SER instead of the BER. This is because usually people don't mention the bit to symbol mapping they used, although it is always assumed to be the gray code, but still it might not be unique, so best to forget about the bit to symbol mapping is to only consider the number of correctly decoded symbols, so if I use a certian transmission technique with bit-to-symbol mapper A and u used another transmission technique & another bit-to-symbol mapper B, our SER results are still comparable but our BERs are not.

Also Linduska pointed out for me that sometimes people are more interested to use SNR rather than EbN0. He said the SNR is useful when one uses pilot symbols and for pilot symbols one can not say how much power is paid per bit because such pilot symbols don't carry bits, so when one considers results in the coherent case for comparison, then it is better to use SNR.
_____________________-
"`Differential space-time block codes from amicable orthogonal designs"' by Zhonglin Chen is a good paper to use when considering transmission of amplitude carrying symbols like QAM/APSK symbols like that of Tao.

From Linduska's meetings, he mentioned I think that Radon is the one who opened the area of OSTBC to extend Alamouti's code for multiple antennas. This is also mentioned in "A Four Transmit Antenna Orthogonal Space-Time Block Code with Full Diversity and Rate" for Lori saying that Radon showed that complex orthogonal designs can not achieve full diversity and rate simultaneously for all symbol constellations, except in the two antennas (Alamouti;s case) case. In the introduction of this 2-page paper, Lori clearly stated that one cannot achieve orthogonality, full diversity & full rate for any signal constellation for M>2 Tx antennas. I believe that the code introduced by Chau Yuen in "Single symbol decodable differential space time modulation based on QO-STBC", he used a full rate, full diversity & Orthogonal STBC for M=4 & M=8 Tx antennas by imposing conditions on the constellation. His paper is very nice & worth rereading, he showed all steps in reaching the proposed constellation.
OOO look at this :), In Lori's paper he emphasized my understanding that Radon's condition was meant to say one cannot achieve orthogonality, full diversity & full rate for any signal constellation, but if we impose certain constraints on the constellation, we can achieve orthogonal full rate & full diversity code. Here is his sentence :) " At first, it appears the new code violates the Hurwitz-Radon theorem, which states that such orthogonal designs cannot exist for all possible symbol constellations. However, they do exist for some specific constellations."
Here http://www.ece.tamu.edu/~ldalton/documents/MSthesis.pdf is the Master thesis of Lori Dalton in 2002 about the new orthogonal full rate full diversity code.
In her thesis, she used same convention as me. In page 14, he defined diversity as follows.
"Diversity is a measure of the average number of channels fully utilized by each piece of information transmitted. The maximum diversity available to a space-time system is NtNr, which is the total number of channels between the transmitter and receiver."
Also in your thesis, show with a simple example, that just sending the symbols redundantely over more than one transmit antenna will not result in any gain as is the case with Rx antennas. This was well explained in the Studienarbeit. And the reason was that, in the equation of the received symbols with Rx diversity you see that the different the square of the received symbols add up & the noise adds (without square so it averages out). However with Tx diversity, both signals & noise add without sqaure so the signal can add destructively. Hence, Tx diversity is not as easy as Rx diversity, and the transmit signal needs some structure to gurantee that the different versions of the received symbols add up.
___
In page 6 of Lori's thesis, I like her explaination about diversity & coding gain, where she not only just explained it in a figure but also mathematically, showing that the diversity order represents the slope of the BER curve and the coding gain as a shift of the curve along the x-axis, on a logarithmic ordinate scale.
A new piece of information mentioned by Lori, is "A necessary, but insufficient, condition for full diversity is that each symbol must be transmitted over every antenna.", for example check page 31 where the STTD-OTD code is ingenearl having a diversity order of 2, since each symbol is transmitted only over two antennas.
Another performance criterion is the determinant criterion, which addresses coding gain. For full diversity schemes, it simply maximizes the minimum determinant of S-S', where as for -let's call them- diversity defficient schemes, the coding gain is defined as the minimum product of all non-zero eigenvalues (unlike the determinant which is the product of all eigenvalues), one can define the product of all non-zero eigenvalues as defined by Hughes as ||+
__Also note in Lori's MS page 15, where she clarified the use of Hochwald's definition of diversity product saying that it can be used only in the case of square matrices, otherwise we must use the determinant of another square matrix like (S-S')H (S-S') as used by most other authors since it works fine with rectangular matrices S of dimension TxM where T not equals M. However, so far I found no way to use the rectangular matrices in Differential transmission. So I may also use Hochwald's definition for the coding gain.
___
As done by Loris in her Master thesis. It is very good to include the MRC curve for performance of the system using one transmit antenna & M receive antennas, as compared to the transmit diversity techniques used with 1 Rx antenna and M Tx antennas. Also remember Alamouti proved that in 2 Tx & 1 Rx antenna with Alamouti's OSTBC results in same performance as 1 Tx & 2 Rx MRC Rx diversity. So you need to do two MRC simulations, one for 2 antennas and one for 4, so as to keep it as a reference. I belive that is even more important in terms of comparison more than comapring with coherent case, since the 3dB difference will always be there I believe regardless the Tx diversity technique used. Where as, the curve for same number of Rx antennas as that of number of Tx antennas in the STBC, we have a reference to compare between the different techniques, or probably a lower limit to see how far are we from the best we can do.
___
one simple reminder that spectral efficiency is defined as Bitrate/BW in units of bits/s/Hz. You may also use R for the code rate defined as R=K/T, and use may be eita as used by lori since it is the symbol of efficiency for the spectral efficiency.
__
Lori'd thesis p.18, again why Tx diversity & not the easy Rx diversity >>cost.
As I understand, Orthogonal codes are most remarkable for having simple ML receivers that decouple the symbols. [Lori, thesis]
Lori defined the "Hurwitz-Radon" theorem in p.20 & then stated that "Notice both real and complex orthogonal designs only consider linear codes designed
to work for all possible symbol constellations."
You may also pass by the literature review of Lori, and others to give a near-complete literature review about who did what in what is most important to know about in STCs.

tailored=designed
paradigm=namozag

I think it is nice in your thesis to say that the independent symbol detection advantage for Orthogonal STBC, also implies that all symbols can be decoded in parallel. This is mentioned in "Differential space-time block codes from amicable orthogonal designs" by Zhonglin Chen, as follows Thus, it will have linear decoding complexity. Moreover, due
to the property of independent decoding, the detections of the information complex symbols can be carried out in parallel.
_________
While reading paper "A Full-Diversity Rate-One STBC for Four Tx Antennas with Single-Symbol Decoding" (2002), The description is good to be utilized in my documentation. 
- In the detection of the information symbols, it is a big advantage to convert the joint detection of all symbols in one matrix to a single symbol detection. This converts the complexity from exopnential increase with q (Alphabet size=q, so search space is q^K, where K is the number of symbols per transmit matrix, to linear increase with q (search space=q x K). This advantage of single-symbol (simple-nonjoint) decoding is always guranteed in Orthogonal STBC & simultaneously orthogonality gurantees full diversity.
The paper clearly explains single-symbol decoding & double-symbol decoding.
Worth mentioning is the literature review in this paper, but have in mind it is working in the coherent case.
________________________________
Remember the master thesis you found about Differential Space Time codes named Differential Amplitude phase STM_Master_thesis_2004 saved in C:\Local Disk E\C-tech\Master project\papers\STBCs\DSTBC-with amplitude mod
________________________________
http://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=991138
"Differential Modulation Using Space–Time Block Codes"
Girish Ganesan and Petre Stoica 
is a good paper to use. It explains the advantage of using OSTBC in that it decouples the different indeterminants (Xi, i=1>> K) which significantly reduces the decoding complexity. He also refers to different papers which I may use.
The full version of the work of Ganesan & Stoica is in 
"Differential Detection Based on Space-Time Block Codes" in 2002
http://www.springerlink.com/content/ap8bebkc10hju155/fulltext.pdf
_____________________________________
A thing I remebered now & like to remind myself of.
Hochwald proved that if a code design is good in the coherent case, it will also be good for the non-coherent case. May be that's why both have the same rank & determinant design criteria. 
_____________________________
It is also worth mentioning that the transmission of real symbols can lead to a rate one code (I know for upto 8 Tx antennas). The transmission of real symbols is explained in 
The full version of the work of Ganesan & Stoica is in 
"Differential Detection Based on Space-Time Block Codes" in 2002
http://www.springerlink.com/content/ap8bebkc10hju155/fulltext.pdf
____________________________________________
Note that he determinant rule that I use a lot 
det (I+AB)=det(I+BA) is called  Sylvester's determinant theorem  
I got this information from Wikipedia
http://en.wikipedia.org/wiki/Determinant
So that that as you also stated the name of the matrix inversion lemma
_______________________________________
of course explain the difference between the coding gain & the diversity gain with an illustrative figure.
____
need not be = mesh shart ykoon
we can do without= momken nestaghna 3an (double check it)
____________________________-
An important note.
In Hochwald's DUSTM, and in DOSTBC, & probably also other schemes. If you compare the curves for different number of transmit antennas (M) you see that you gain only at the high SNR range. This is due to diversity, the slope gets higher which indicates that two curves of different M will intersect at a point, below which is the lower M curve better, and above which is the higher M curve better. A basic reason is that when we defined the design criteria based on the PEP, we worked it out in the high SNR range which is in some applications the range of interest.
Also note that in the paper of Xue-Bin Liang in the paper "Unitary Signal Constellations for Differential Space-Time Modulation with Two transmit antennas: Parametric codes, Optimal Designs and bounds", he defined two different parameteres for the constellation design, the first is the diversity sum which is to be maximized for a good performance in the low SNR range, and the other is the diversity product which is to be maximized for a good performace in the high SNR range.
In all the codes that have been used in this thesis, we used the diversity product (or also known as the coding gain) as the design criteria. That's why we only see gain at the high SNR range, but loss at the low SNR range. 

If we call the point at which we start to gain in performance as SNR threshold or Eb/N0 threshold, then we see that this threshold increases ( which means the starting SNR after which we gain is shifted to the right), by increasing the spectral efficiency. 
This is clear when comparing the two curves of DUSTM with 1 bits/channel use (SNR threshold is at 5 dB) and 2 bits/channel use (SNR threshold is at 15 dB).
Also note that this SNR threshold point is a common point when comparing any two different M curves. 

Q: what is the SNR range of interest in the current applications
_________________________________________________________
When comparing with a coherent curve, always mentioned under "perfect" channel estimation.
____________________________________________________________
Decoding of Differential OSTBC with Non-Unitary Constellations using multiple Received Data blocks-2010 is a good reference for MSDD in MIMO systems using OSTBCs. Examine references 5 to 8 that use M-QAM modulation in OSTBC. I only know that of Tarokh and Tao.
Also see paper [10]"Differential Coding for Non-Orthogonal Space-Time Block Codes with Non-Unitary Constellations over Arbitrarily Correlated Rayleigh Channels" for the same authors. It is really a must read paper, it is done in 2009 with all the lterature review, nicely it was comparing their approach with the mear-optimal approach of Tao in DOSTBC with QAM signals saying they acheived better performance with a different approach.  Also nicely they show a different technique that achieves a 1 dB gain compared to that of Chau Yuen that is based on QOSTBC. Note that one of the authors have done his PhD in Differential Space-Time Codes. I may explore their two papers, to see this technique & examine the theory of using MSDD in MIMO. 
WOW [10] is using a non-coherent detection scheme similar to the GLRT scheme, which starts with a coherent ML receiver, then replaces the channel H by the optimal analytical estimate of it (by differentiating the metric and equating it to zero), then it substitutes this estimate back to the ML metric. This can be described as joint channel and symbol detection. In the SISO case using GLRT results in reduced complexity compared to the ML mertic. Here using the approach similar to the GLRT technique, the error performance is improved.
Also [10] has shown that the golden code is 5 dB superior than the QOSTBC of Chau Yuen
__________________________________________________________________
Make sure you adjusted the headers in the way you like. I like to have a header with the chapter name on one page and the section name on the opposite page.
____
for QOSTBC See ``A Simple Differential Modulation Scheme for Quasi-Orthogonal Space-Time Block Codes with Partial Transmit Diversity''...As lori this is how they explained diversity ``This code has rate one, but
diversity order two, since each symbol passes through only two of the four transmit antennas.``Page 2 left down
_________
I believe it is necessary to make it clear that the fading coefficients remain fixed within a frame and changes \emph{independently} from one frame to the next.
__ Don't forget to mention the rate diversity trade off.
__
include at the end the conclusion highlighting the main principles used all over the thesis and include the future challenges.
__
Include an Abstract which summerizes the thesis concern helping the reader to decide whether or not reading it is of interest.
In the PhD [11], a nice explaination of the advantages of noncoherent detection is explained in page 29. You may also add..For an MxN MIMO system, coherent systems need to estimation MN channel coefficients resulting in an increased overhead and complexity. Moreover the estimated channel coefficient may be inaccurate,,,
It is also good to clearly define noncoherent systems, where the is no CSI at both communication ends. Differential modulation is one possible way of achieveing noncoherent communications.
Also section 1.2 page 30 is very well written, I have a similar goal and I need to include this as well in the introduction.
It is VERY good to highlight the goals to be achieved in a STC scheme like in [11, p.31]. And mention that these aspects (complexity, spectral efficiency, diversity order, and error rate)
I like the scientific style used in [11], I want to adopt a similar style in the rest and most important part of the thesis.
_
In explaining diversity you can say it alternatively (may be in the abstract or introduction). In receive diversity, if the receiver is equipped with N receive antennas,it  ideally posses N independent observations of the same transmitted signal
__
It is also good to mention somewhere that in the context of the thesis, decoding and detection are used interchangeably with no meaning difference.
Also mention that the system is a low pass domain complex system
__
Note that I have always seen that the used expression to describe the channel is not as Rayleigh flat fading channel but flat Rayleigh fading channel, also matlab help uses this notation for example frequency-flat rayleigh fading channel. In such a channel, the channel coefficients vary independently from one frame to the next.
__
Unitray transmission refers to the case when the signals transmitted over any  antenna as a function of time is of unit energy and is orthogonal to all signals transmitted on the other antennas
__
incorporates=yedmeg in arabic
__
I have seen this in like 2 papers .Differential space-time block encoding entails an expansion of the constellation of the symbols that are differentially encoded.
For example, when binary phase shift keying (BPSK) messages are encoded by (10), the elements of() will form a certain 5-PAM constellation which contains the symbols
However, it can be verified that at any time, the total energy transmitted is unity. Similarly, when 4-PSK messages are encoded, the elements of.. will be 9-QAM (quadrature
amplitude modulation). see page 2 in [21].
Since in Rayleigh block fading channel, the channel is constant within a frame, this implies that the chanel remains constant within a window length of N symbols
__You may also say block fading Rayleigh channel or fast fading Rayleigh channel...

I finally got an answer to the question of how to say the complexity increases expoenentially in..... It is mentioned in the phD [19] that for example if the complexity increases with M^(N), then we say that the complexity increases exponentially with (in) N. see [19, p.54 pdf]
__
This is how Matlab help explains the reason behind uzsing quasi-static Rayleigh fading channels ... 
Quasi-Static Channel Modeling


Typically, a path gain in a fading channel changes insignificantly over a period of 1/(100fd) seconds, where fd is the maximum Doppler shift. Because this period corresponds to a very large number of bits in many modern wireless data applications, assessing performance over a statistically significant range of fading entails simulating a prohibitively large amount of data. Quasi-static channel modeling provides a more tractable approach, which you can implement using these steps.
This I got from the help page entitled ''Fading Channels".. because at very small doppler shifts relative to teh symbol rate, the channel changes insiginifcantly over a long duration also explained by matlab in the smae help page, in section `More About the Quasi-Static Technique`"
Use the notation of Monte Carlo simulations with some littel explanation of the term

_________
In [22] Non-Coherent Sphere Decoding for Space-Time Modulation by Vincent Hag in Feb 2005... a very well written master thesis..a very good source for documentation in SISO and MIMO case
It is also important to mention that improveing the transmission in the downlink is of importance since mostly a user downloads more data than that uploaded. See page.12 in [22]. Include this in your thesis
__
In your introduction define well the purpose of the thesis. Inspired by noncoherent detection for simplicity, improvement of performance by modulating the bits not only over the phase llike PSK and Unitary STCs but also over the amplitude like DAPSK and non-unitary STCs. The conventional way for detecting the transmitted information noncooherently (w.o channel knowledge) is by processing two consecutive receive blocks (or symbols in SISO case). This Conventional Differential Detection (CDD) is however inferior to coherent detection by about 3 dB. Additionally, the CDD results in an error florr in fast fading channels. To bridge the gap between the performance of coherent detectors and non coherent ones, and also to better learn about the fading statistics and remove the error floor in Fast fas'ding channels, processing more than 2 received blocks (Multiple-(Super)Symbol detection) has been studied in several papers. 
__
The main goals for any STC scheme is to achieve maximum rate, full diversity, minimum decoding complexity, minimum decoding latency and good error rate performance.
__
define j to be the imaginary unit somewhere
__
in the first time where you defined Eb/N0 in your thesis, specify that it is the energy per information bit.
__
Note that I have two notation problems , with N and D_s. In STC I am using D_ll' for the distance matrix.
___
if you have the time , replace eqnarrays which have a compound form of equations (not a derivation of an equation) with aligning, so that the numbers of the equation be placed in the middle, see eq (5.2)
__
in your small sized BER curves, you may increase the legend font size further.
__
remove the numbering from unreferenced equations
_
consider a list of symbols if time permits
notify that the same symbols might signify different meanings in the siso and mimo chapters
__ 
SISO abbreviation is used in SISO table of metrics, so if you won't define it in introduction, then just define it in SISO chapter.
_________print all pages with a figure to make sure they are clear even with a black and white version.
_______Into and conclusion is the most important of all chapters as they will be most read for a quick investigation. Make them as motivating, to the point with a good and clear scientific description as possible.
___Acknowedgement 
__Check E_b/N_0 is written this way and not Eb/N0 in the figures x label.

==> List_of_Symbols.tex <==
List of Symbols
M
N
Y
S
V
j 
L
q
f_d
t
tau
omega
D_ll'
G
H


==> MSDD_MIMO.tex <==
Increasing the observation window above (beyond) two blocks in the conventional differential detection, has the effect of reducing the performance loss gap of the noncoherent BER curves compared to coherent ones and additionally suppresses the error floor encountered in fast fading channels.
You will find a very good illustration of MSDD in the PhD dissertation in  [19]
[21] is a very good reference talking about MSDD in STCs and providing a nice summery for the history of STCs
%Sphere decoding is explained in the book u have, use it for simple introduction of the concept

==> Notations2.tex <==
\chapter*{Notations list}

\newsym{\Cd}{C_D}
          {Depletion layer capacitance}

\newsym{\Cm}{C_m}
          {MOS capacitance per unit area}

\newsym{\Cox}{C_{ox}}
          {Oxide capacitance, $\Cox = \eSiO2/\dox$}

\newsym{\Cs}{C_S}
          {Semiconductor capacitance per unit area}

\otherdef[\CS]{\Cs}
          {Pipeline cell storage capacitor}


\addcontentsline{toc}{chapter}{Notations List}

==> SISO_figs.tex <==

% In explaining the canonical form of a candidate sequence for PSK detection, say like in [20] section 3.2.1

% % See Hochwald's interpretation of GLRT in "systematic design of unitary Space-Time Constellations`` p.1964
% \section{DPSK}
% \label{s:DPSK}
% Simulation results for DPSK
% \begin{figure}[htp]
%   \centering
% 	\includegraphics[width=0.8\textwidth , trim= 2cm 0 1cm 0]{DPSK_AWGN} %trim option's parameter order: left bottom right top
% 	\caption{Multiple-symbol detection of DPSK over an AWGN channel}
% 	\label{fig:DPSK_AWGN}
% 	\end{figure}
% 	
% \begin{figure}[htp]
%   \centering
% 	\includegraphics[width=0.8\textwidth, trim=1cm 0cm 1cm 0]{DPSK_Rayleigh_block_fading} 
% 	\caption{Multiple-symbol detection of DPSK over a Rayleigh block fading channel}
% 	\label{fig:DPSK_RBF} % I will use RBF as the ID of Rayleigh Block fading & RFF as that of Rayleigh Fast Fading
% 	\end{figure}
% 	
%	\newpage	
%\section{DAPSK}
%\label{s:DAPSK}
%
%Ring Ratio search
%\begin{figure}[htp]
%  \centering
%		\subfloat[Ring ratio search for 2DPSK-4DASK]{\label{subfig:2DPSK_4DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_2DPSK_4DASK}}                
%  	\subfloat[Ring ratio search for 4DPSK-2DASK]{\label{subfig:4DPSK_2DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_4DPSK_2DASK}}
%  \caption{Ring ratio test for 8DAPSK}
%  \label{fig:ring_ratio_8DAPSK}
%\end{figure}
%
%\begin{figure}[htp]
%  \centering
%		\subfloat[Ring ratio search for 2DPSK-8DASK]{\label{subfig:2DPSK_8DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_2DPSK_8DASK}}                
%  	\subfloat[Ring ratio search for 4DPSK-4DASK]{\label{subfig:4DPSK_4DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_4DPSK_4DASK}}\\
%    	\subfloat[Ring ratio search for 8DPSK-2DASK]{\label{subfig:8DPSK_2DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_8DPSK_2DASK}}
%  \caption{Ring ratio test for 16DAPSK}
%  \label{fig:ring_ratio_16DAPSK}
%\end{figure}
%
%\begin{figure}[htp]
%  \centering
%		\subfloat[Ring ratio search for 2DPSK-16DASK]{\label{subfig:2DPSK_16DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_2DPSK_16DASK}}                
%  	\subfloat[Ring ratio search for 4DPSK-8DASK]{\label{subfig:4DPSK_8DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_4DPSK_8DASK}}\\
%    	\subfloat[Ring ratio search for 8DPSK-4DASK]{\label{subfig:8DPSK_4DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_8DPSK_4DASK}}
%      	\subfloat[Ring ratio search for 16DPSK-2DASK]{\label{subfig:16DPSK_2DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_16DPSK_2DASK}}
%  \caption{Ring ratio test for 32DAPSK}
%  \label{fig:ring_ratio_32DAPSK}
%\end{figure}
%
%\begin{figure}[htp]
%  \centering
%		\subfloat[Ring ratio search for 4DPSK-16DASK]{\label{subfig:4DPSK_16DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_4DPSK_16DASK}}                
%  	\subfloat[Ring ratio search for 8DPSK-8DASK]{\label{subfig:8DPSK_8DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_8DPSK_8DASK}}\\
%    	\subfloat[Ring ratio search for 16DPSK-4DASK]{\label{subfig:16DPSK_4DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_16DPSK_4DASK}}
%      	\subfloat[Ring ratio search for 32DPSK-2DASK]{\label{subfig:32DPSK_2DASK_ring_ratio}\includegraphics[width=0.5\textwidth]{Ring_ratio_search_awgn_32DPSK_2DASK}}
%  \caption{Ring ratio test for 64DAPSK}
%  \label{fig:ring_ratio_64DAPSK}
%\end{figure}
%
%\newpage
%Ring Ratio Influence
%
%
%\begin{figure}[htp]
%  \centering
%	\subfloat[Ring ratio influence for 8DAPSK]{\label{subfig:8DAPSK_ring_inf}\includegraphics[width=0.5\textwidth]{Ring_ratio_influence_8DAPSK}}     \subfloat[Ring ratio influence for 16DAPSK]{\label{subfig:16DAPSK_ring_inf}\includegraphics[width=0.5\textwidth]{Ring_ratio_influence_16DAPSK}}\\
%  \subfloat[Ring ratio influence for 32DAPSK]{\label{subfig:32DAPSK_ring_inf}\includegraphics[width=0.5\textwidth]{Ring_ratio_influence_32DAPSK}}
%  \subfloat[Ring ratio influence for 64DAPSK]{\label{subfig:64DAPSK_ring_inf}\includegraphics[width=0.5\textwidth]{Ring_ratio_influence_64DAPSK}}
%  \caption{Ring ratio influence for M-DAPSK}
%  \label{fig:ring_influence_DAPSK}
%\end{figure}
%
%%%%% Figures of the BER for DAPSK in the different channels
%\newpage
%Simulation results for DAPSK
%\begin{figure}[htp]
%  \centering
%	\subfloat[8DAPSK over AWGN]{\label{subfig:8DAPSK_AWGN}\includegraphics[width=0.6\textwidth]{8DAPSK_AWGN}}\\
%	\subfloat[16DAPSK over AWGN]{\label{subfig:16DAPSK_AWGN}\includegraphics[width=0.6\textwidth]{16DAPSK_AWGN}}
%	\label{fig:DAPSK_AWGN:part1}
%	\caption[]{}
%\end{figure}
%	
%	\begin{figure}
%	\ContinuedFloat
%	\centering
%	\subfloat[32DAPSK over AWGN]{\label{subfig:32DAPSK_AWGN}\includegraphics[width=0.6\textwidth]{32DAPSK_AWGN}}
%	\caption{BER curves for DAPSK Multiple-symbol detection over an AWGN channel}
%	\label{fig:DAPSK_AWGN:part2}
%	\end{figure}
%
%\begin{figure}[htp]
%  \centering
%	\subfloat[8DAPSK over Rayleigh block fading channel]{\label{subfig:8DAPSK_RBF}\includegraphics[width=0.6\textwidth]{8DAPSK_Rayleigh_Block_Fading}}\\
%	\subfloat[16DAPSK over Rayleigh block fading channel]{\label{subfig:16DAPSK_RBF}\includegraphics[width=0.6\textwidth]{16DAPSK_Rayleigh_Block_Fading}}
%	\caption[]{}
%	\label{fig:DAPSK_Rayleigh_Block_Fading:part1}
%	\end{figure}
%	
%	\begin{figure}
%	\ContinuedFloat
%	\centering
%	\subfloat[32DAPSK over Rayleigh block fading channel]{\label{subfig:32DAPSK_RBF}\includegraphics[width=0.6\textwidth]{32DAPSK_Rayleigh_Block_Fading}}
%	\caption{BER curves for DAPSK Multiple-symbol detection over a Rayleigh block fading channel}
%	\label{fig:DAPSK_Rayleigh_Block_Fading:part2}
%	\end{figure}
%	
%	\begin{figure}[htp]
%  \centering
%	\subfloat[8DAPSK over Rayleigh fast fading channel]{\label{subfig:8DAPSK_RFF}\includegraphics[width=0.6\textwidth]{8DAPSK_Rayleigh_Fast_Fading}}\\
%	\subfloat[16DAPSK over Rayleigh fast fading channel]{\label{subfig:16DAPSK_RFF}\includegraphics[width=0.6\textwidth]{16DAPSK_Rayleigh_Fast_Fading}}\\
%	\label{fig:DAPSK_Rayleigh_Fast_Fading:part1}
%	\caption[]{}
%	\end{figure}
%	
%	\begin{figure}
%	\ContinuedFloat
%	\centering
%	\subfloat[32DAPSK over Rayleigh fast fading channel]{\label{subfig:32DAPSK_RFF}\includegraphics[width=0.6\textwidth]{32DAPSK_Rayleigh_Fast_Fading}}
%	\caption{BER curves for DAPSK Multiple-symbol detection over a Rayleigh fast fading channel at $f_{D}\!\times\! T_{s}= 0.02$}
%	\label{fig:DAPSK_Rayleigh_Fast_Fading:part2}
%	\end{figure}
%	

==> STBC_Fast_Fading.tex <==
\chapter{Fast fading case}
%Probably I won't include specific work for the fast fading case, but let's hope we will.
In the best case, if there is any useful insight in the metric proved by Linduska for the fast fading case, I may include his lengthy (yet useful) proof and explain such useful insights.
I may also include the simulations -I still haven't run them yet, but hopefully I will soon- that use the metric proved for RBF in the RFF case. In this case may be it will make sense to include such a chapter.
I may show the performance degradation of using the RBF in the RFF channel as a function of fdTs, and compare it to the case of (hopefully) using the RFF channel metric.
In [15] page 5 , "Figures 8 and 9 show results for a time-varying channel with a normalized maximum Doppler frequency of fdTs = 0.01. Here, the channel is not exactly constant during transmission of two successive matrices which results in increased estimation errors for the effective channel parameters and in a performance degradation of the differential detector." This is to say why performance degradation is expected when using the metric proved for RBF in RFF channel. Bauch said in the last sentence of the paper that the approach of differential amplitude and unitary STM (Approach of Xia) outperfoms all other schemes in the paper in the case of fast fading channel. mm interesting

==> description.tex <==
%---------------------------------------------------------------------------%
% description.tex
%---------------------------------------------------------------------------%
% student
\set{author}     {Rania, Morsi} %<-- Vor- und Zuname Student
\set{street}     {} %<-- Adresse
\set{city}       {} %<-- Wohnort
\set{field}      {Communications Technology} %<-- Z.B. Communications Technology
\set{studentid}  {693530} %<-- Matrikelnummer
\set{birthday}   {}
\set{email}      {rania.morsi@uni-ulm.de}

% thesis number
\set{thesisno}   {01} %<-- Laufende Nummer für Bibliothek

% supervisor
\set{svIname}    {Dipl.-Ing. Alexander Linduska}
\set{svIinitials}{al}
\set{svIroomno}  {43.2.238}
\set{svIemail}   {alexander.linduska@uni-ulm.de}
% in case of external thesis
%\set{svEname}    {Dipl.-Ing. Tobias Wolff}
%\set{svEinitials}{dz} % Offizieller interner Betreuer (cf. official_supervisor)
%\set{svEcompany} {Harman/Becker Automotive Systems GmbH}
%\set{svEphone}   {(0731) 3994 369}
%\set{svEemail}   {twolff@harmanbecker.com}

% examiners (siehe auch organisation.tex!!!)
\set{examinerA}  {Prof.\ Dr.-Ing.\ J.\ Lindner}
\set{examinerB}  {}

% the dates [Verwaltung]
\setdate{start}  {15}{05}{2010} %<-- Offizielle Anmeldung
\setdate{finish} {15}{11}{2010} %<-- Offizielle Abgabe
\setdate{talk}   {22}{11}{2010} %<-- Vortragstermin
\setdate{rating} {30}{11}{2010} %<-- Termin Erstgutachten

%% !!! The following line is NOT just a comment
%% it serves as OPTIONS for dsthesis class
%%
% DOCUMENT_OPTIONS =  master,intern,english,e-technik

% options:
% diplarb/studarb/master/bachelor - default: diplarb für Diplomarbeiten
% erasmus                - for ERASMUS students
% german/english	 - language
% intern/extern          - default: intern
% e-technik/informatik   - defines field of study for registration

%---------------------------------------------------------------------------%

\set{title}{Investigations on Increased Data Rate Differential Space-Time Block Codes for Single Carrier Wireless Systems}
\set{description}{%
For achieving high spectral efficiency in wireless transmission systems, channel knowledge at least at
the receiver is required to retrieve the information transmitted. Transmission schemes which rely on 
full channel state information (CSI) are called {\sl coherent}. Obtaining full CSI is performed by using channel
measurement techniques like pilot assisted or blind channel measurement schemes. A reasonable constraint for
using coherent transmission schemes is a large coherence time of the channel, e.~g. the channel has to stay
(approximately) constant for a long time. In some applications this constraint is not guaranteed or it is not
intended to spend complexity for channel measurement. If the channel coherence time is long enough 
(but of course much shorter than in the case of coherent transmission) it is still possible to transmit
information without full CSI at the receiver. Suitable transmission techniques for this case are so 
called {\sl differential transmission schemes}. Differential phase shift keying (DPSK) is a long known 
technique for single carrier systems using one transmit antenna, which has a penalty of about \unit[3]{dB} compared
with its coherent counterpart. Improving the performance for differential transmission led to multisymbol
detection schemes for DPSK as well as to differential amplitude phase shift keying (DAPSK). A further
improvement was the development of differential modulation techniques for multiple input multiple output
(MIMO) systems.\\[0.2cm]
In the first part of this master thesis, a short comparison of different differential modulation techniques for
single transmit antenna systems should be provided. The results and insights obtained hereby shall be used
in the second part for enhancing the concepts of differential modulation to MIMO systems. 
In the second part existing differential MIMO techniques should be compared and the possibility of developing
new schemes evaluated.
}
 \set{requirements}{%
   $\bullet$ Lectures NT I+II, AWIMUC\\
  $\bullet$ MATLAB-Knowledge}

%---------------------------------------------------------------------------%


==> papers_STC_draft.tex <==
%Papers Draft 
[1] S. Alamouti, A simple transmit diversity technique for wireless communications,"
Selected Areas in Communications, IEEE Journal on, vol. 16, pp. 1451 {1458, oct.
1998.
[2] V. Tarokh, N. Seshadri, and A. R. Calderbank, "Space-time codes for
high data rate wireless communication: Performance criteria and code
construction," IEEE Trans. Inform. Theory, Mar. 1998.
[3] Tarokh, V.; Jafarkhani, H. & Calderbank, A. Space-time block codes from orthogonal designs Information Theory, IEEE Transactions on, 1999, 45, 1456 -1467
[4] Radon, J. Lineare scharen orthogonaler matrizen Abhandlungen aus dem Mathematischen Seminar der Universität Hamburg, Springer Berlin / Heidelberg, 1922, 1, 1-14
[5]Tarokh, V. & Jafarkhani, H. A differential detection scheme for transmit diversity Selected Areas in Communications, IEEE Journal on, 2000, 18, 1169 -1174
[6] Hochwald, B. & Marzetta, T. Unitary space-time modulation for multiple-antenna communications in Rayleigh flat fading Information Theory, IEEE Transactions on, 2000, 46, 543 -564
[7] Hochwald, B. & Sweldens, W. Differential unitary space-time modulation Communications, IEEE Transactions on, 2000, 48, 2041 -2052
[8] Hughes, B. Differential space-time modulation Information Theory, IEEE Transactions on, 2000, 46, 2567 -2578
[9] Bhatnagar, M. & Hjø andrungnes, A. Decoding of Differential OSTBC with Non-Unitary Constellations Using Multiple Received Data Blocks Communications (ICC), 2010 IEEE International Conference on, 2010, 1 -5
[10] Bhatnagar, M.; Hjorungnes, A. & Song, L. Differential coding for non-orthogonal space-time block codes with non-unitary constellations over arbitrarily correlated rayleigh channels Wireless Communications, IEEE Transactions on, 2009, 8, 3985 -3995
[11] Outage Probability in a Multi-Cellular Network Using Alamouti Scheme
[12] Tao, M. & Cheng, R. Differential space-time block codes Global Telecommunications Conference, 2001. GLOBECOM '01. IEEE, 2001, 2, 1098 -1102 vol.2
[13] Tarokh, Differential Space Time Block Codes Using Nonconstant Modulus Constellations, Nov 2003
[14] Chen, Z.; Zhu, G.; Shen, J. & Liu, Y. Differential space-time block codes from amicable orthogonal designs Wireless Communications and Networking, 2003. WCNC 2003. 2003 IEEE, 2003, 2, 768 -772 vol.2
[15] Bauch, G. & Mengi, A. Non-unitary orthogonal differential space-time modulation with non-coherent soft-output detection Vehicular Technology Conference, 2005. VTC-2005-Fall. 2005 IEEE 62nd, 2005, 2, 977 - 981
[16] Jafarkhani, H. A quasi-orthogonal space-time block code Wireless Communications and Networking Conference, 2000. WCNC. 2000 IEEE, 2000, 1, 42 -45 vol.1
[17] Yuen, C.; Guan, Y. L. & Tjhung, T. T. Quasi-orthogonal STBC with minimum decoding complexity: further results Wireless Communications and Networking Conference, 2005 IEEE, 2005, 1, 483 - 488 Vol. 1
[18] An 8x8 Quasi-Orthogonal STBC Form for Transmissions over Eight or Four Antennas. Rohan Grover, Weifeng Su, and Dimitris A. Pados.
http://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=4712691
[19] PhD_Techniques for noncoherent space-time communications by Riediger 2006
[20] Application of sphere decoding to MSDD by Lutz Lampe, Robert Schober.. section 3.2.1
[21] Multiple-Symbol Differential Detection for Space-Time Block Codes by Gao 2002
[22] Non-Coherent Sphere Decoding for Space-Time Modulation... a very well written master thesis..good source for documentation



A paper on MSDD for diagonal STM using DF-DD and MSDSD
http://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=01006558


==> presentation_points.tex <==
So welcome to you all. As said my master thesis is about space-time coding which is the science of transmit diversity using multiple transmitting antennas. We will show the investigation of these codes in the differential domain.

Slide outline: So the presentation will go as follows
first I'll quickly show the use of differential modulation in single antenna systems, the so-called SISO systems
Then I'll switch to differential modulation in multiple antenna systems, the so-called (MIMO) systems.
In this the design criteria of space-time codes will be explained
then we will show the theoretical analysis and simulation results of three different space-time coding schemes in the differential domain.

 Slide 2:
So why differential. Well, Differential modulation schemes are just one type of non-coherent transmission, where the receiver does not need channel knowledge for the detection process.\\
This alleviates the need of channel estimation, which has several disadvantages
First it is difficult to continuously track the channel in a fast varying environment
channel estimation also introduces overhead which reduces the useful data rate
